RSVP for VPSA : A Meta Design Study on Rapid Suggestive Visualization Prototyping for Visual Parameter Space Analysis

Visual Parameter Space Analysis (VPSA) enables domain scientists to explore input-output relationships of computational models. Existing VPSA applications often feature multi-view visualizations designed by visualization experts for a specific scenario, making it hard for domain scientists to adapt them to their problems without professional help. We present RSVP, the Rapid Suggestive Visualization Prototyping system encoding VPSA knowledge to enable domain scientists to prototype custom visualization dashboards tailored to their specific needs. The system implements a task-oriented, multi-view visualization recommendation strategy over a visualization design space optimized for VPSA to guide users in meeting their analytical demands. We derived the VPSA knowledge implemented in the system by conducting an extensive meta design study over the body of work on VPSA. We show how this process can be used to perform a data and task abstraction, extract a common visualization design space, and derive a task-oriented VisRec strategy. User studies indicate that the system is user-friendly and can uncover novel insights.

==> sections/030_Meta-Design-Study/design-space-table.tex <==
\begin{table}[t]
 \caption{\label{tab:design-space}Visualization options in the derived design space}
\centering
 \begin{tabular}{||c|l l||} 
 \hline \hline
& \textbf{Visualization Options} & \textbf{Abbr}. \TBstrut\\ 
 \hline\hline
 \multirow{7}{*}{\rotatebox[origin=c]{90}{Parameter}}& \histfull & \hist \Tstrut\\ 
 &\spfull & \sp \\
 &\splomfull & \splom \\
 &\rsplomfull & \rsplom \\
 &\pscfull & \psc \\
 &\pcfull & \pc \\
 &\dcpfull & \dcp \Bstrut\\
 \hline \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{CO}} & \coIlinefull & \coIline \Tstrut\\
 & \coIhistfull & \coIhist \\
 & \coIboxfull & \coIbox \Bstrut\\
 \cline{2-3}
 & \coIIgridfull & \coIIgrid \Tstrut\\ 
 & \coIIjuxfull & \coIIjux \\
 & \coIIsupfull & \coIIsup \Bstrut\\
 \hline \hline
 
 \end{tabular}

\end{table}		

==> sections/050_Evaluation/case-study-I-old.tex <==
\subsection{Case Study: Crystal Powder Diffraction (OLD!!)}
\label{sec:case-study}
\label{sec:case-study-I}
%
Our case-study user is a physics professor who specializes in solid-state materials.
He studies crystalline structures using a procedure known as \emph{powder diffraction} and compares the results to simulated model data using $\chi^2$ (see \autoref{eq:chi2} to learn about molecular behavior inside the crystal.
The knowledge gained from such experiments helps the physicist to grow new crystals with desired features.  
For this case study, the physicist provided fifty random samples of a 4D parameter space along with 1D outputs and derived $\chi^2$-metrics. 
%The following case study took approximately 1.5 hours.

The domain expert received the same brief introduction to the tool as the participants from the usability study.
After the introduction, the user started his session by loading his data into RSVP. 
%The user then dragged the input parameters onto the appropriate selection fields and observed how his selection affected the various visualizations in the overview section. 
%He was interested to see how switching the ${\chi}^2$-marker between the various encoding channels changed the visualizations.
%
After some initial experimentation with data selections and studying visualizations in the overview, he began to familiarize himself with the guidance tasks and was interested to see which visualizations were recommended for which task. 
%He tried different combinations just to see how the ranking and the according score would get adjusted. 
He copied several of the suggested visualizations into the application area, arranged them and started interacting with the data.
During the next twenty minutes, he experimented with the various visual encodingy offered by the system, tried different arrangements and settings for these encodings and was genuinely interested in how they interacted with each other.
%\begin{figure}[t]
%\centering
%  \includegraphics[width=\linewidth]{images/powder_screenshot.png}
%  \caption{Example of an interactive visualization composed during the case study on the X-Ray diffraction dataset. Showcased are a scatterplot matrix of the input space and the performance graphs outputted by the diffraction model. Two specific parameter settings are highlighted for closer inspection. }
%  \label{fig:powder_screenshot}
%\end{figure}
% The domain scientist was impressed by the speed provided by the tool and the possibility to experiment with different ideas in real-time. 
% Reflecting on his experience on a previous design study, he wished that he would have had such a tool back then.

%One thing that has to be specifically be mentioned is his original skepticism about the recommendations provided by the system.
%Eventually he wanted to know how the recommendation worked and we explained briefly, that it is basically a number of how often this visualization has been used in applications crafted by visualization experts when they had to tackle one of those tasks. 
%This is when he eventually became less skeptical and more interested about the score.

%He still had a problem though with the first recommendation we encountered, when we chose optimization in the recommendation pane.
%The top recommendations for this task were histograms with a score of 9 and parallel coordinates with a score of 8.5; 
%In his mindset, using histograms on the provided input parameters would only show him how well the random sampling on these parameters was performed.
%While this is actually true, it was explained to him how histograms could be used in combination with other visualizations to explore certain details about the dataset.
%Unfortunately, due to a bug in the tool while the case study was performed, the histograms could not be copied into the staging area and the interaction with other visualizations could not be tested.
%For this reason, we came up with an alternative solution to mimic the behavior of the histograms through parallel coordinates. 
%We dragged all the input parameters onto the Dims area, encoded the ${\chi}^2$ as color and copied this to the staging area.
%Then, we changed the orientation of the parallel coordinates from left-to-right to top-to-bottom and choose symbols for markers instead of lines. 
%Now, the density of the symbold would basically show how high a histogram bar would be in a certain position.
%Additionally, we aligned the the filters with axes of the parallel coordinates, so we could filter according to range.

%A screenshot of this experiment taken during the study is shown in figure~\ref{fig:case_study_2_2}

%\begin{figure}[t]
%\centering
%  \includegraphics[width=8cm]{images/case_study_2_2.jpg}
% \caption{Screenshot taken during case study}
 % \label{fig:case_study_2_2}
%\end{figure}

%\begin{figure}[ht]
%\centering
%  \includegraphics[width=8.5cm]{images/awesome_recommendation.png}
%  \caption{Recommendation of the recommendation primer chosen for the tasks during our case study, confirming the likings of our domain scientist}
%  \label{fig:awesome_recommendation}
%\end{figure}

The most notable part of the case study was the following event.
The domain scientist was interested in a recommendation for the tasks optimization, fitting, sensitivity and outliers.
He encoded the four input parameters as spatial dimensions and the quality metric ${\chi}^2$ as color, as suggested by the tool.
He also encoded the 1D object showing the diffraction patterns as Function Graphs. 
The recommended visualizations were a Scatterplot Matrix to provide an overview and to find outliers and Parallel Coordinates to analyze sensitive regions in the parameter setting. 
For the 1D object, the tool recommended the Function Graphs and the Cumulative Histogram.
Within a few minutes, he created the visualization represented in Figure \ref{fig:case-study-powder-app}.

\begin{figure}[h]
\centering
  \includegraphics[width=7.4cm]{images/RSVP_Case_Study_Powder.png}
  \caption{Parallel Coordinates, arranged from top to bottom and filtered to emphasize values with a low ${\chi}^2$. The visualization reveals that $angl1$ and $angl2$ have little influence on the quality of the ${\chi}^2$-result.}
  \label{fig:case-study-powder-app}
\end{figure}

%This finding was very interesting to him.
It can easily be seen that on axis \emph{angl1}, the values to obtain a good ${\chi}^2$-measurement are scattered, then they become narrower for \emph{zoff1}, wider again for \emph{angl2} and narrower again for \emph{zoff2}.
This basically means that \emph{angl1} and \emph{angl2} have little to no influence to get a good ${\chi}^2$-result, whereas \emph{zoff1} and \emph{zoff2} do. 
Although known to the domain expert, he had originally gained this insight through long computational cycles. 
He had to run a Levenberg-Marquardt optimization algorithm on his model for hours until the algorithm would finally converge to a single parameter set. 
The problem for the optimization algorithm probably was the fact that \emph{angl1} and \emph{angl2} had too little influence on the final result, thus making it impossible for the algorithm to come up with a single perfect parameter setting. 
The variance in these two axes was expressed as uncertainty values, which the scientist had to make sense of over weeks of work.
In comparison, he was impressed that he could get the same information from a rather simple visualization and a set of fifty randomly sampled parameter settings - something that he never deemed possible.
%The Function Graphs turned out to be not very helpful, but according to the user, this was not surprising. 
%
The user expressed his interest in using this tool for his further research, especially to see if these findings hold true for even higher-dimensional parameter spaces.

\begin{itemize}
    \item possibly mention that for the visualization of the 3D-molecules they used \st{Igor} CrystalMaker. 
    \item \TODO{Ask Chuck if this is still the case}{and why they use it in the first place}{}
\end{itemize}

==> sections/050_Evaluation/qri.tex <==
\subsection{Qualitative Result Inspection}
\label{sec:qri}

Our general approach described in \autoref{sec:meta-design-study} aims at creating a visualization design space that is both minimalistic and expressive. 

\paragraph*{Meeting the Requirements}

\paragraph*{Design Goal }

==> sections/060_Discussion/snippets/reverse-engineered.tex <==
The interesting finding is not the visualization recommendation per se, but the fact that it could actually be reverse-engineered from a body of work over that topic.


==> sections/060_Discussion/validity.tex <==
\subsection{Validity of our approach}
\label{sec:validity}

In both case studies, the domain experts were able to confirm existing knowledge (CS1) or preconceived notions (CS2) about their models. 
The interesting insight from CS1
They did not question their findings and believed that VPSA is a valid approach to analyze input-output-oriented models.

\point{The confirmation of preconceived notions about their data helped to build trust in both the VPSA-strategy and the RSVP system. 
The accompanying realizations about their models }


\point{On \visrec}
While other solutions presented in \visrec are often based on crowd-sourced opinions about the effectiveness for certain visualizations (e.g. \cite{Wongsuphasawat2016a, Moritz2019}, our recommendaiton strategy is based on peer-reviewd solutions, devised by visualization experts.

\tempsec{paragraph*}{Vis-expert perspective}
From the perspective of a visualization expert, our proposed design space might appear rather simple.
We have two arguments for that. 
First, we did not invent this design space, but we derived it from a pre-defined set of criteria.
Second, visualization experts are not the targeted user group, but domain experts are, which might only have very limited visual literacy \cite{Russell2016, Wong2019}

\tempsec{subsubsection*}{Possible complaints}
\point{Your design space is too simple}
\point{Your recommendation strategy is too simple}
\point{Your complex objects are too simple}
